Experimental Study of Periodically Poled Piezoelectric Film Lithium Niobate Resonator at Cryogenic Temperatures

This work reports the first study of periodically poled piezoelectric film (P3F) lithium niobate (LiNbO3) resonators at cryogenic temperatures. We experimentally investigate the temperature dependency of resonant frequencies and quality factor (Q) of higher-order Lamb modes up to 20 GHz between 80{\deg}K and 297{\deg}K, using a tri-layer P3F LiNbO3 resonators as the experimental platform. The supported thickness-shear Lamb modes between second-order symmetric (S2) and eleventh-order antisymmetric (A11) modes show temperature coefficients of frequency (TCF) averaging -68.8 ppm/K. Higher Q and more pronounced spurious modes are observed at lower temperatures for many modes. Upon further study, the cryogenic study will be crucial for identifying dominant loss mechanisms and origins of spurious modes in higher-order Lamb wave devices for millimeter-wave applications.

==> IMS_modify_IEEEtran_18b_CTAN_V7.tex <==
% IMS_modify_IEEEtran_18b_CTAN_V5.tex
%         created by Causal Productions Pty Ltd, 
%	  http://www.causalproductions.com
%	  info@causalproductions.com
%
%	  This file is Copyright 2017-2019 Causal Productions Pty Ltd.
%	  Permission is granted to use this file and its associated files
%	  for conferences for which Causal Productions has been contracted
%	  to prepare the conference proceedings.
%
% This file contains format modifications to the standard IEEE style file
% called IEEEtran.cls version 1.8b, as hosted on CTAN at the following URL:
%	http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
%
% The purpose of the format modifications is to implement a paper format
% traditionally used by IMS conferences, which differs from the standard
% IEEE conference paper format in various ways, such as font sizes.
%  
% This file is NOT intended to be used with the different IEEEtran.cls version 1.8
% that is distributed by IEEE at the following URL:
%	http://www.ieee.org/web/publications/pubservices/confpub/AuthorTools/conferenceTemplates.html
% Despite having the same version number 1.8, the CTAN and IEEE versions are
% different and this particular modification file is designed only for the 
% CTAN version.
%
% HISTORY
% 20180920 V3 first release for review
% 20181009 V3c no change, version number bumped to match paper template file
% 20191020 V4c changed section heading number-name spacing so that it is specified individually for
%               section - use a fixed space between number and name
%               subsection - make the name align with paragraph indentation
%               subsubsection - make the name align with paragraph indentation
%               paragraph - make the name align with paragraph indentation
% 20201028 V5 no change, version number bumped to match paper template file
%          V6 was never created, as V6 template was a version generated by IMS 2023 organizers
% 20231206 V7 no change, version number bumped to match paper template file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter

\def\@IMSauthorblockNAMEstyle{\normalfont\IMSauthorsize}
\def\@IMSauthorblockAFFILstyle{\normalfont\IMSaffilsize}
\def\@IMSauthorblockEMAILstyle{\normalfont\IMSaffilsize}
%
\def\IMSauthorblockNAME#1{%
\relax\@IMSauthorblockNAMEstyle%
#1%
}%
\def\IMSauthorblockAFFIL#1{%
\relax\@IMSauthorblockAFFILstyle%
\vskip\@IEEEauthorblockAtopspace
#1%
}%
\def\IMSauthorblockEMAIL#1{%
\relax\@IMSauthorblockEMAILstyle%
\vskip\@IEEEauthorblockAtopspace
#1%
}%
%
\newcommand{\IMSauthor}[1]{%
\ifIsBlindReviewVersion%
\author{\phantom{\parbox{\textwidth}{\center\relax#1}}}%
\else%
\author{\parbox{\textwidth}{\center\relax#1}}%
\fi%
}%
%
\newif\ifIsBlindReviewVersion
\def\IMSthispaperforblindreview{\IsBlindReviewVersiontrue}
\def\IMSthispaperforfinalpublication{\IsBlindReviewVersionfalse}
%
%
%
% IMS: override title block font sizes
% formats the Title, authors names, affiliations and special paper notice
% THIS IS A CONTROLLED SPACING COMMAND! Do not allow blank lines or unintentional
% spaces to enter the definition - use % at the end of each line
\def\@maketitle{\newpage
\bgroup\par\addvspace{0.5\baselineskip}\centering%
\ifCLASSOPTIONtechnote% technotes
   {\bfseries\large\@IEEEcompsoconly{\sffamily}\@title\par}\vskip 1.3em{\lineskip .5em\@IEEEcompsoconly{\sffamily}\@author
   \@IEEEspecialpapernotice\par{\@IEEEcompsoconly{\vskip 1.5em\relax
   \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par
   \hfill\@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
\else% not a technote
   \vskip0.2em{\IMStitlesize\ifCLASSOPTIONtransmag\bfseries\LARGE\fi\@IEEEcompsoconly{\sffamily}\@IEEEcompsocconfonly{\normalfont\normalsize\vskip 2\@IEEEnormalsizeunitybaselineskip
   \bfseries\Large}\@title\par}\vskip1.0em\par% CAUSAL PRODUCTIONS change on this line
   % V1.6 handle \author differently if in conference mode
   \ifCLASSOPTIONconference%
      {\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
       \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par}\relax
   \else% peerreviewca, peerreview or journal
      \ifCLASSOPTIONpeerreviewca
         % peerreviewca handles author names just like conference mode
         {\@IEEEcompsoconly{\sffamily}\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
          \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par
          {\@IEEEcompsoconly{\vskip 1.5em\relax
           \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par\hfill
           \@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
      \else% journal, peerreview or transmag
         \ifCLASSOPTIONtransmag
            % transmag also handles author names just like conference mode
            % it also uses \@IEEEtitleabstractindextex, but with one line less
            % space above, and one more below
           {\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
            \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par
           {\vspace{0.5\baselineskip}\relax\@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\vspace{-1\baselineskip}\par}}\relax
         \else% journal or peerreview
           {\lineskip.5em\@IEEEcompsoconly{\sffamily}\sublargesize\@author\@IEEEspecialpapernotice\par
           {\@IEEEcompsoconly{\vskip 1.5em\relax
            \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par\hfill
            \@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
         \fi
      \fi
   \fi
\fi\par\addvspace{0.0\baselineskip}\egroup}% CAUSAL PRODUCTIONS change on this line, reduce the vspace from 0.5\baselineskip to 0.0

% IMS: change font sizes in the document
%	paper title is 24pt
%	bib items are 9pt 
%	author names are 11pt
%	author affils are 10pt
%	captions of figs and tables are 9pt
\def\IMStitlesize{\@setfontsize{\IMStitlesize}{18}{21pt}}% CAUSAL PRODUCTIONS change on this line
\def\IMSauthorsize{\@setfontsize{\IMSauthorsize}{12}{13pt}}% CAUSAL PRODUCTIONS change on this line
\def\IMSaffilsize{\@setfontsize{\IMSaffilsize}{12}{13pt}}% CAUSAL PRODUCTIONS change on this line
\def\IMScaptionsize{\@setfontsize{\IMScaptionsize}{8}{9pt}}% CAUSAL PRODUCTIONS change on this line
\def\IMSbibsize{\@setfontsize{\IMSbibsize}{8}{9pt}}% CAUSAL PRODUCTIONS change on this line

\def\@IEEEauthorblockNstyle{\IMSauthorsize\@IEEEcompsocnotconfonly{\sffamily}\@IEEEcompsocconfonly{\large}}%CAUSAL PRODUCTIONS removed sublargesize to get correct IMSauthorsize
\def\@IEEEauthorblockAstyle{\IMSaffilsize\@IEEEcompsocnotconfonly{\sffamily}\@IEEEcompsocconfonly{\itshape}\@IEEEcompsocconfonly{\large}}%CAUSAL PRODUCTIONS removed normalsize to get correct IMSaffilsize
% The default if the user does not use an author block
\def\@IEEEauthordefaulttextstyle{\IMSauthorsize\@IEEEcompsocnotconfonly{\sffamily}\sublargesize}%CAUSAL PRODUCTIONS

\def\thebibliography#1{\section*{\refname}%
    \addcontentsline{toc}{section}{\refname}%
    % V1.6 add some rubber space here and provide a command trigger
    \IMSbibsize\@IEEEcompsocconfonly{\small}\vskip 0.3\baselineskip plus 0.1\baselineskip minus 0.1\baselineskip% CAUSAL PRODUCTIONS change on this line
    \list{\@biblabel{\@arabic\c@enumiv}}%
    {\settowidth\labelwidth{\@biblabel{#1}}%
    \leftmargin\labelwidth
    \advance\leftmargin\labelsep\relax
    \itemsep \IEEEbibitemsep\relax
    \usecounter{enumiv}%
    \let\p@enumiv\@empty
    \renewcommand\theenumiv{\@arabic\c@enumiv}}%
    \let\@IEEElatexbibitem\bibitem%
    \def\bibitem{\@IEEEbibitemprefix\@IEEElatexbibitem}%
\def\newblock{\hskip .11em plus .33em minus .07em}%
% originally:
%   \sloppy\clubpenalty4000\widowpenalty4000%
% by adding the \interlinepenalty here, we make it more
% difficult, but not impossible, for LaTeX to break within a reference.
% IEEE almost never breaks a reference (but they do it more often with
% technotes). You may get an underfull vbox warning around the bibliography, 
% but the final result will be much more like what IEEE will publish. 
% MDS 11/2000
\ifCLASSOPTIONtechnote\sloppy\clubpenalty4000\widowpenalty4000\interlinepenalty100%
\else\sloppy\clubpenalty4000\widowpenalty4000\interlinepenalty500\fi%
    \sfcode`\.=1000\relax}

% IMS: make a version of \@makecaption which uses \IMScaptionsize
%	and which formats all figure captions as justified if long, centered if short,
%	and formats all table captions using identical format to figure captions.
%	We are discarding the archaic small-caps format of table captions which was so hard to read.
%
\long\def\@makecaption#1#2{%
% test if is a for a figure or table
%  if figure, must make a vertical space before caption to separate caption from figure content
%  if table, must make a vertical space after caption to separate caption from table content
\ifx\@captype\@IEEEtablestring%
\par\@IEEEtabletopskipstrut% strut used to align table caption with facing column
\else
\@IEEEfigurecaptionsepspace
\fi
% 20180920 use IMScaptionsize, use two nonbreaking spaces, not one
\setbox\@tempboxa\hbox{\normalfont\IMScaptionsize {#1.}\nobreakspace\nobreakspace #2}%
\ifdim \wd\@tempboxa >\hsize%
% if caption is longer than a line, let it wrap around
\setbox\@tempboxa\hbox{\normalfont\IMScaptionsize {#1.}\nobreakspace\nobreakspace}%
\parbox[t]{\hsize}{\normalfont\IMScaptionsize\noindent\unhbox\@tempboxa#2}%
% if caption is shorter than a line, center if conference, left justify otherwise
\else
\ifCLASSOPTIONconference \hbox to\hsize{\normalfont\IMScaptionsize\hfil\box\@tempboxa\hfil}%
\else \hbox to\hsize{\normalfont\IMScaptionsize\box\@tempboxa\hfil}%
\fi\fi
% test if is a for a figure or table
%  if figure, must make a vertical space before caption to separate caption from figure content
%  if table, must make a vertical space after caption to separate caption from table content
\ifx\@captype\@IEEEtablestring%
\@IEEEtablecaptionsepspace
\else
\fi}

% IMS: define table-caption-to-table separation separately from figure-to-figure-caption separation
\newlength\tablecaptiontotableskip
\newlength\figuretocaptionskip
% but only \abovecaptionskip is used above figure captions and *below* table
% captions
\setlength\tablecaptiontotableskip{0.5\baselineskip}% 0.5bs gives about 3mm from caption baseline to table
\setlength\figuretocaptionskip{0.0\baselineskip}% 0bs gives about 3mm from figure to caption top of lc letters, which matches appearance of table.
\def\@IEEEfigurecaptionsepspace{\vskip\figuretocaptionskip\relax}%
\def\@IEEEtablecaptionsepspace{\vskip\tablecaptiontotableskip\relax}%

% IMS: Use Michael Shells suggested fix to reduce the space around emdash following Abstract and Index Terms headings
\def\abstract{\normalfont%
\@IEEEabskeysecsize\bfseries\textit{\abstractname}\,\bfseries\textit{---}\,%
\@IEEEgobbleleadPARNLSP}%
\def\endabstract{\relax\vspace{0ex}\par%
\normalfont\normalsize}%

\def\IEEEkeywords{\normalfont%
\@IEEEabskeysecsize\bfseries\textit{\IEEEkeywordsname}\,\bfseries\textit{---}\,%
\@IEEEgobbleleadPARNLSP}%
\def\endIEEEkeywords{\relax\vspace{0.67ex}%
\par\if@twocolumn\else\endquotation\fi%
\normalsize\normalfont}%


%%%%%
% Define \IMSauthorrefmark to allow more flexible marking than the \IEEEauthorrefmark command
% The refmarks can now be a string of any length, of any characters.
\DeclareRobustCommand*{\IMSauthorrefmark}[1]{\raisebox{0pt}[0pt][0pt]{\textsuperscript{\footnotesize{#1}}}}%
%
% CAUSAL PRODUCTIONS: No extra space between title and authors
\def\@IEEEauthorblockNtopspace{0ex}
% CAUSAL PRODUCTIONS: 1mm extra space between author names and affiliations
\def\@IEEEauthorblockAtopspace{1mm}
%
%%%%%%%%%%%%%%%%%%%%%%
%
\setlength{\columnsep}{6.3mm}% IMS
\def\tablename{Table}% IMS: was TABLE in IEEETran, but we are now using capitalized caption text not smallcaps
\def\thetable{\arabic{table}}% IMS: Tables are numbered using arabic not roman
\def\IEEEkeywordsname{Keywords}% use Keywords instead of Index Terms
%
%%%%%%%%%%%%%%%%%%%%%%
%
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
{0.7ex plus .5ex minus 0ex}{\normalfont\normalsize\itshape}}%
%
%%%%%%%%%%%%%%%%%%%%%%
%
\setlength{\parindent}{1.5em}% make the default para indent larger to match WORD template
%
% 20191023 we remove the V3c indentation of section headings to match paragraph indentation, 
% and revert to the original IEEE section heading style without spacing, and the spacing is
% now done individually for the 4 levels, below.
\def\@seccntformat#1{\csname the#1dis\endcsname\relax}% moved the spacer \hskip 0.5em to individual handlers below
%
% The following are copied from IEEEtran.cls line 2585 and modified here
\def\thesectiondis{\thesection.\hskip 0.5em}%					I.	% CAUSAL PRODUCTIONS: moved the hskip spacer from \@seccntformat to here
\def\thesubsectiondis{{\hbox to\parindent{\Alph{subsection}.}}}%		B.	% CAUSAL PRODUCTIONS: indent the subsection name to match paragraph indent
\def\thesubsubsectiondis{{\hbox to \parindent{\arabic{subsubsection})}}}%	3)	% CAUSAL PRODUCTIONS: indent the subsubsection name to match paragraph indent
\def\theparagraphdis{{\hbox to \parindent{\alph{paragraph})}}}%			d)	% CAUSAL PRODUCTIONS: indent the subsubsubsection name to match paragraph indent
%
% now we redefine the list indents so they take the new value of \parindent
\IEEEilabelindentA \parindent
\IEEEilabelindent \IEEEilabelindentA
\IEEEelabelindent \parindent
\IEEEdlabelindent \parindent
\IEEElabelindent \parindent
%%%%%%%%%%%%%%%%%%%%%%

\newlength\@IMSparindent
\setlength{\@IMSparindent}{\parindent}

\newcommand\IMSdisplayacksection[1]{%
\ifIsBlindReviewVersion%
%\noindent\phantom{\parbox[t]{\columnwidth}{\normalbaselines\setlength{\parindent}{\@IMSparindent}#1\strut}}%\IMSacktext
\noindent\phantom{\parbox[t]{\columnwidth}{\normalbaselines\setlength{\parindent}{\@IMSparindent}{#1}\strut}}%\IMSacktext
\else%
\noindent\parbox[t]{\columnwidth}{\normalbaselines\setlength{\parindent}{\@IMSparindent}{#1}\strut}%
\fi%
}%

%%%%%%%%%%%%%%%%%%%%%%

\makeatother


